Data Quality in Edge Machine Learning: A State-of-the-Art Survey

Data-driven Artificial Intelligence (AI) systems trained using Machine Learning (ML) are shaping an ever-increasing (in size and importance) portion of our lives, including, but not limited to, recommendation systems, autonomous driving technologies, healthcare diagnostics, financial services, and personalized marketing. On the one hand, the outsized influence of these systems imposes a high standard of quality, particularly in the data used to train them. On the other hand, establishing and maintaining standards of Data Quality (DQ) becomes more challenging due to the proliferation of Edge Computing and Internet of Things devices, along with their increasing adoption for training and deploying ML models. The nature of the edge environment -- characterized by limited resources, decentralized data storage, and processing -- exacerbates data-related issues, making them more frequent, severe, and difficult to detect and mitigate. From these observations, it follows that DQ research for edge ML is a critical and urgent exploration track for the safety and robust usefulness of present and future AI systems. Despite this fact, DQ research for edge ML is still in its infancy. The literature on this subject remains fragmented and scattered across different research communities, with no comprehensive survey to date. Hence, this paper aims to fill this gap by providing a global view of the existing literature from multiple disciplines that can be grouped under the umbrella of DQ for edge ML. Specifically, we present a tentative definition of data quality in Edge computing, which we use to establish a set of DQ dimensions. We explore each dimension in detail, including existing solutions for mitigation.

==> assets/figures/tikz/bias-types.tex <==
\tikzset{%
    parent/.style  = {%
            draw, rounded corners=2pt, text width=3cm,
            align=center, font=\sffamily, rectangle,
            inner sep=.1cm, fill=blue!20
        },
    root/.style   = {parent, rounded corners=2pt, thin, align=center, fill=green!30},
    child/.style = {parent, thin, rounded corners=2pt, align=center, fill=pink!60,},
    gchild/.style = {parent, thin, rounded corners=2pt, align=left, fill=green!30, align=center, text width=4cm},
    g2child/.style = {parent, thin, align=left, fill=yellow!30, align=center},
    edge from parent/.style={draw=black, edge from parent fork left}
}
\begin{forest} for tree={%
    grow=east,
    growth parent anchor=west,
    parent anchor=east,
    child anchor=west,
    calign=center,
    edge path={%
    \noexpand\path[\forestoption{edge},->, >={latex}]
    (!u.parent anchor) -- + (10pt,0pt) |-  (.child anchor) \forestoption{edge label};
    }
    }
    % l sep is used for arrow distance
    [Bias, parent,  l sep=10mm,
    [User bias, child, l sep=10mm,
            [Historical bias, gchild],
            [Population bias, gchild],
            [Self-selection bias, gchild],
            [Social bias, gchild],
            [Behavioral bias, gchild],
            [Temporal bias, gchild]
        ],
    [Algorithm bias, child, l sep=10mm,
            [Algorithmic bias, gchild],
            [User interaction bias, gchild, l sep=10mm,
                    [Ranking bias, g2child],
                    [Presentation bias, g2child]
                ],
            [Popularity bias, gchild],
            [Emergent bias, gchild],
            [Evaluation bias, gchild]
        ],
    [Data bias, child, l sep=10mm,
            [Measurement bias, gchild],
            [Ommitted variable bias, gchild],
            [Representation bias, gchild],
            [Aggregation bias, gchild,
                    [Simpsom's paradox, g2child],
                    [Modifiable areal unit problem, g2child]
                ],
            [Sampling bias, gchild],
            [Longitudinal data fallacy, gchild],
            [Linking bias, gchild],
        ]
    ]
\end{forest}

==> assets/figures/tikz/byzantine-taxonomies.tex <==
% \tikzset{%
%   parent/.style={align=center,text width=3cm,rounded corners=3pt},
%   child/.style={align=center,text width=3cm,rounded corners=3pt}
% }
% \begin{forest}
%   for tree={
%   % forked edges,
%   draw,
%   rounded corners,
%   node options={align=center,},
%   text width=2.7cm,
%   },
%   where level=0{%
%   }{%
%   folder,
%   grow'=0,
%   if level=1{%
%   before typesetting nodes={child anchor=north},
%   edge path'={(!u.parent anchor) -- ++(0,-5pt) -| (.child anchor)},
%   }{},
%   }
%   [LMS, fill=gray!25, parent
%     [Funktionale \\Anforderungen, for tree={fill=brown!25, child}
%         [Lerninhalte organisieren]
%         [Lerninhalte erstellen]
%         [Lerninhalte abfragen]
%         [Kommunikation]
%         [Benutzerkonten\-führung]
%         [Steuerungs\-funktionen]
%     ]
%     [Nicht-Funktionale Anforderungen, for tree={fill=red!25,child}
%         [Zuverl{\"a}ssig\-keit]
%         [Skalierbar\-keit und Effizienz]
%         [Benutzer\-freundlich\-keit]
%         [Portierbarkeit]
%         [Datenschutz / Informationssicherheit]
%         [Erweiterbar\-keit]
%         [Anpassbarkeit]
%     ]
%     [Technische Rahmen\-bedinungen, for tree={fill=blue!25, child}
%         [System\-architektur]
%         [Software\-kriterien]
%         [Schnittstellen]
%         [Wartung und Support
%             [Support\-leistungen]
%             [Software-Pflege]
%         ]
%     ]
%   ]
% \end{forest}


% TiKz code from: https://shantoroy.com/latex/Draw-literature-survey-tree-in-latex/
\tikzset{%
  parent/.style  = {%
      draw, rounded corners=2pt, text width=3cm,
      align=center, font=\sffamily, rectangle,
      inner sep=.1cm, fill=blue!20
    },
  root/.style   = {parent, rounded corners=2pt, thin, align=center, fill=green!30},
  child/.style = {parent, thin, rounded corners=2pt, align=center, fill=pink!60,},
  gchild/.style = {parent, thin, rounded corners=2pt, align=left, fill=green!30, align=center},
  g2child/.style = {parent, thin, align=left, fill=yellow!30, align=center},
  edge from parent/.style={draw=black, edge from parent fork left}
}
\begin{forest} for tree={%
  % grow'=south,
  % growth parent anchor=north,
  % parent anchor=south,
  % child anchor=north,
  % calign=center,
  % edge path={%
  % \noexpand\path[\forestoption{edge},->, >={latex}]
  % (!u.parent anchor) -- + (10pt,0pt) |-  (.child anchor) \forestoption{edge label};
  % }
  }
  % l sep is used for arrow distance
  [Classifications of\\ Byzantine attacks, align=center, base=bottom,
  [Target-based, edge label={node[midway,left,font=\scriptsize]{test}},
      [Model poisoning]
        [Data poisoning]%
    ]
    [Objective-based,
      [Targeted]
        [Untargeted]%
    ]
  ]
\end{forest}







% \begin{tikzpicture}
%   [level distance=3cm,
%     level 1/.style={sibling distance=12cm},
%     level 2/.style={sibling distance=6cm},
%     level 3/.style={sibling distance=3cm}
%   ]
%   \tikzstyle{bag} = [align=center]
%   \tikzset{every tree node/.style={align=center,anchor=north}}
%   % \tikzset{level distance=2cm, sibling distance=5cm}
%   \node (Root)  {Parle couramment?}
%   child {
%       node {Comprend?}
%       child {
%           node {Peut répéter?}
%           child {node[bag] {Aphasie\\globale} edge from parent node[left] {Non }}
%           child {node[bag] {Aphasie\\transcorticale\\mixte} edge from parent node[right] {Oui }}
%           edge from parent node[left] {Non}
%         }
%       child {
%           node {Peut répéter?}
%           child {node[bag] {Aphasie\\de Broca} edge from parent node[left] {Non }}
%           child {node[bag] {Aphasie\\transcorticale\\motrice} edge from parent node[right] {Oui }}
%           edge from parent node[right] {Oui}
%         }
%       edge from parent node[left] {Non}
%     }
%   child {
%       node {Comprend?}
%       child {
%           node {Peut répéter?}
%           child {node[bag] {Aphasie\\de Wernicke} edge from parent node[left] {Non }}
%           child {node[bag] {Aphasie\\transcorticale\\sensorielle} edge from parent node[right] {Oui }}
%           edge from parent node[left] {Non}
%         }
%       child {
%           node {Peut répéter?}
%           child {node[bag] {Aphasie\\de conduction} edge from parent node[left] {Non }}
%           child {node[bag] {Aphasie\\anomique} edge from parent node[right] {Oui }}
%           edge from parent node[right] {Oui}
%         }
%       edge from parent node[right] {Oui}
%     };

% \end{tikzpicture}

==> assets/figures/tikz/noise-tree.tex <==
\begin{tikzpicture}
  [level distance=3cm,
    level 1/.style={sibling distance=12cm},
    level 2/.style={sibling distance=6cm},
    level 3/.style={sibling distance=3cm}
  ]
  \tikzstyle{bag} = [align=center]
  \tikzset{every tree node/.style={align=center,anchor=north}}
  % \tikzset{level distance=2cm, sibling distance=5cm}
  \node (Root)  {Does \(\mathcal{Y} = \tilde{\mathcal{Y}}\)?}
  child {
      node {Does \(\tilde{y}_{i}\) depend on \(y_{i}\)?}
      child {
          node {Does \(\tilde{y}_{i}\) depend on \(X_{i}\)?}
          child {node[bag] {Aphasie\\globale} edge from parent node[left] {No }}
          child {node[bag] {Aphasie\\transcorticale\\mixte} edge from parent node[right] {Yes }}
          edge from parent node[left] {No}
        }
      child {
          node {Does \(\tilde{y}_{i}\) depend on \(X_{i}\)?}
          child {node[bag] {Aphasie\\de Broca} edge from parent node[left] {No }}
          child {node[bag] {Aphasie\\transcorticale\\motrice} edge from parent node[right] {Yes }}
          edge from parent node[right] {Yes}
        }
      edge from parent node[left] {No}
    }
  child {
      node {Does \(\tilde{y}_{i}\) depend on \(y_{i}\)?}
      child {
          node {Does \(\tilde{y}_{i}\) depend on \(X_{i}\)?}
          child {node[bag] {Aphasie\\de Wernicke} edge from parent node[left] {No }}
          child {node[bag] {Aphasie\\transcorticale\\sensorielle} edge from parent node[right] {Yes }}
          edge from parent node[left] {No}
        }
      child {
          node {Does \(\tilde{y}_{i}\) depend on \(X_{i}\)?}
          child {node[bag] {Aphasie\\de conduction} edge from parent node[left] {No }}
          child {node[bag] {Aphasie\\anomique} edge from parent node[right] {Yes }}
          edge from parent node[right] {Yes}
        }
      edge from parent node[right] {Yes}
    };

\end{tikzpicture}

==> assets/figures/tikz/oldtax.tex <==
% TiKz code from: https://shantoroy.com/latex/Draw-literature-survey-tree-in-latex/
\tikzset{%
    parent/.style  = {%
            draw, rounded corners=2pt, text width=3cm,
            align=center, font=\sffamily, rectangle,
            inner sep=.1cm, fill=blue!20
        },
    root/.style   = {parent, rounded corners=2pt, thin, align=center, fill=green!30},
    child/.style = {parent, thin, rounded corners=2pt, align=center, fill=pink!60,},
    gchild/.style = {parent, thin, rounded corners=2pt, align=left, fill=green!30, align=center},
    g2child/.style = {parent, thin, align=left, fill=yellow!30, align=center},
    edge from parent/.style={draw=black, edge from parent fork left}
}
\begin{forest} for tree={%
    grow=east,
    growth parent anchor=west,
    parent anchor=east,
    child anchor=west,
    calign=center,
    edge path={%
    \noexpand\path[\forestoption{edge},->, >={latex}]
    (!u.parent anchor) -- + (10pt,0pt) |-  (.child anchor) \forestoption{edge label};
    }
    }
    % l sep is used for arrow distance
    [Data Quality, parent,  l sep=10mm,
    [\nameref{sub:security_concerns}, child,  l sep=10mm,
    [\nameref{ssub:privacy}, gchild, l sep=10mm
    [\nameref{par:homomorphic_encryption}, g2child]
    [\nameref{par:differential_privacy}, g2child]
    [\nameref{par:privacy:fl}, g2child]
    ]
    [\nameref{ssub:trust_worthiness}, gchild, l sep=10mm,
    [\nameref{par:authentication}, g2child]
        [\nameref{par:reputation_mechanisms}, g2child]
        [\nameref{par:byzantine_fault_tolerance}, g2child]
    ]
    ]
    [\nameref{sub:learning_concerns}, child,  l sep=10mm,
    [\nameref{ssub:niid}, gchild, l sep=10mm,
            [\nameref{par:niid:fl}, g2child]
                [\nameref{par:niid:fedavg}, g2child]
                [\nameref{par:oodg}, g2child]
        ]
        [\nameref{ssub:missing_labels}, gchild, l sep=10mm,
            [\nameref{par:semi_supervised}, g2child]
                [\nameref{par:few_shot}, g2child]
                [\nameref{par:transfer_learning}, g2child]
        ]
    ]
    ]
\end{forest}

==> assets/figures/tikz/taxonomy.tex <==
% TiKz code from: https://shantoroy.com/latex/Draw-literature-survey-tree-in-latex/
\tikzset{%
  parent/.style  = {%
      draw, rounded corners=2pt, text width=3cm,
      align=center, font=\sffamily, rectangle,
      inner sep=.1cm, fill=blue!20
    },
  root/.style   = {parent, rounded corners=2pt, thin, align=center, fill=green!30},
  child/.style = {parent, thin, rounded corners=2pt, align=center, fill=pink!60,},
  gchild/.style = {parent, thin, rounded corners=2pt, align=left, fill=green!30, align=center},
  g2child/.style = {parent, thin, align=left, fill=yellow!30, align=center},
  edge from parent/.style={draw=black, edge from parent fork left}
}
\begin{forest} for tree={%
  grow'=east,
  growth parent anchor=west,
  parent anchor=east,
  child anchor=west,
  calign=center,
  edge path={%
  \noexpand\path[\forestoption{edge},->, >={latex}]
  (!u.parent anchor) -- + (10pt,0pt) |-  (.child anchor) \forestoption{edge label};
  }
  }
  % l sep is used for arrow distance
  [Data Quality, parent,  l sep=10mm,
  [Collection, child, l sep=10mm,
      [Inaccuracy, gchild]
        [Missing Data, gchild]%
    ]
    [Transmission, child, l sep=10mm,
      [Intentional, gchild, l sep=10mm,
          [Data Poisoning, g2child]%
        ]
        [Unintentional, gchild, l sep=10mm,
          [Data Loss (Missing or Incomplete Data), g2child]
            [Data Alteration (Inaccuracy), g2child]%
        ]%
    ]
    [Processing, child, l sep=10mm,
      [Incompleteness, gchild]
        [Inaccuracy, gchild]%
    ]
    [Storage, child, l sep=10mm,
      [Unreliablitity, gchild]
        [Capacity, gchild]%
    ]
    [Training, child, l sep=10mm,
      [Non-\glsxtrshort{abb:iid} data, gchild]
        [Data drift, gchild]%
    ]
    [Byzantine Nodes, child]%
  ]
\end{forest}

==> data-quality/dimensions.tex <==
\subsection{Data quality dimensions}%
\label{sub:data_quality_dimensions}

It follows from \Cref{princple:performance_is_dq} that
the \emph{best} dataset \(\xi\) produces the \emph{best}
(or Bayes-optimal) model i.e., \(\hat{\theta}_{\xi} = \theta^{\ast}\).
More generally, a \emph{good} dataset is one that produces a \emph{good} model
i.e., \(\hat{\theta}_{\xi} \approx \theta^{\ast}\).
Early works on the theory of \gls{abb:ml}~\cite{%
  vapnikPrinciplesRiskMinimization1991,%
  neweyChapter36Large1994,%
  vapnikNatureStatisticalLearning2010%
}
have provided theoretical guarantees for this to be the case
under certain fairly general conditions
on the hypothesis class \(\mathcal{H}\) and the parameter space \(\Theta\).
More precisely, they have shown that, with high probability,
a large enough dataset \(\xi\), drawn \gls{abb:iid}
from the true distribution \(\Pr_{(X, Y)}\),
will produce a good model (in the sense defined above).

This already gives us three sufficient conditions for a dataset to be good,
namely that it is:
\begin{enumerate*}[label=(\roman*)]
  \item large enough,
  \item \gls{abb:iid}, and
  \item drawn from the true distribution.
\end{enumerate*}
Size is usually not seen as a data quality issue,
so we will not consider it further.
The other two conditions, however, are of great interest to us,
and can serve as the main axes of our definition of data quality.
Based on the previous analysis,
we can tentatively divide \gls{abb:dq} concerns into the following categories:
\begin{enumerate}
  \item \emph{Data dependence}.
        Which occurs when the elements of \(\xi\) are not independent.
  \item \emph{Distribution mismatch}.
        Which occurs when the elements of \(\xi\)
        do not follow the true distribution \(\Pr_{(X, Y)}\).
        The joint distribution \(\Pr_{(X, Y)}\)
        is characterized by the marginal distribution \(\Pr_{X}\)
        and the conditional distribution \(\Pr_{Y \mid X}\),
        which allows us to distinguish between two types of distribution mismatch:
        \begin{enumerate}
          \item \emph{Attribute skew}.
                Which happens when the sampling process
                is biased towards certain regions of the input space \(\mathcal{X}\).
          \item \emph{Label noise}.
                Which happens when the labeling process is error-prone.
        \end{enumerate}
\end{enumerate}
It is worth noting that the above scenarios are not mutually exclusive.
Distribution mismatch can happen due to a combination
of attribute skew and label noise,
and data dependence is likely to cause attribute skew.

An easy objection one could raise against the above categorization,
and indeed against \Cref{princple:performance_is_dq} itself,
is its reliance on the premise that model quality
can be reduced to performance (i.e., true risk).
In doing so, it fails to completely capture
the context-dependent nature of \gls{abb:dq}.
As a result, all the above considerations
are more or less \emph{intrinsic} to the data.

To justify the inclusion of \emph{extrinsic} considerations,
we argue that model performance is not sufficient to capture model quality.
A model can be considered bad while having excellent performance,
if it fails to satisfy certain ethical or social criteria.
For example, a model that has near-optimal true risk
can have arbitrarily high risk on a certain subset \(A \subset \mathcal{X}\),
if \(\Pr{\left[X \in A \right]}\) is small enough.
Such a model is unfair to the elements of \(A\),
which can lead to legal and ethical issues if \(A\) is a marginalized group.
Similarly, a model that allows for the reconstruction of \(\xi\),
thereby betraying the privacy of the individuals in the training set
is also considered bad, even if it has excellent performance.
Alternatively, the data could be of low quality
due to its source rather than its content.
For example, a dataset that can include deliberately wrong information.
Accounting for these considerations, we amend \Cref{princple:performance_is_dq}
to a more general form.
\begin{principle}\label{princple:mq_is_dq}
  A good dataset \(\xi\) can be defined as one that (when used for \gls{abb:erm})
  produces a good model, which in turn can be defined
  as a model \(\hat{\theta}_{\xi}\) that satisfies certain ethical and social criteria,
  in addition to having low true risk \(\mathcal{R}\left( \hat{\theta}_{\xi} \right)\).
\end{principle}
An extended version of the above taxonomy to include these extrinsic considerations
in compliance with \Cref{princple:mq_is_dq} is shown in \Cref{fig:dq:dims:taxonomy}.
\begin{figure}[hbt]
  \begin{center}
    \resizebox{\linewidth}{!}{\input{assets/figures/tikz/dimensions}}
  \end{center}
  \caption{A taxonomy of data quality dimensions}\label{fig:dq:dims:taxonomy}
\end{figure}



==> fairness/solutions.tex <==
\subsection{Fair edge machine learning}\label{sub:fairness:solutions}

Ensuring fairness in edge \gls{abb:ml} is a vital and challenging task
that has been the subject of much research in recent years.
These efforts can be categorized according to multiple axes,
including the specific \gls{abb:ml} task they target,
the notion of fairness they aim to enforce,
the type of fairness they consider,
and the stage of the learning process at which they intervene.
In this section, we adopt the latter categorization,
presenting examples of solutions that have been proposed
in the literature of fair \gls{abb:ml}, with a focus on edge \gls{abb:fl}.

\subsubsection{Preprocessing}\label{ssub:fairness:solutions:pre}

Data preprocessing is an umbrella term that describes
all operations applied to the data before training.
For the purposes of fairness, these can include
data cleaning~\cite{brunetUnderstandingOriginsBias2019},
data augmentation~\cite{wangNonIIDDataRebalancing2021},
and data transformation~\cite{calmonOptimizedPreProcessingDiscrimination2017}.
In this section, we examine a selection of preprocessing techniques for fair \gls{abb:ml}.
The reader can refer to%
~\cite{wernerdevargasImbalancedDataPreprocessing2023,abhishekMachineLearningImbalanced2023}
for a comprehensive and systematic review of data preprocessing techniques for imbalanced data.

\citet{calmonOptimizedPreProcessingDiscrimination2017}
propose an optimization-based approach to transform a dataset
to ensure demographic parity with respect to a given sensitive attribute.
They formulate the problem as a constrained quasi-convex program
where the objective is to maximize the similarity
between the original and transformed distributions,
subject to the fairness constraint,
and a bound on the distortion of individual data points.
\citet{brunetUnderstandingOriginsBias2019}
on the other hand, propose a data cleaning approach,
where they identify and remove bias-inducing documents from a corpus
for the task of learning word embeddings.

In the contexts of edge \gls{abb:ml} and \gls{abb:fl},
\citet{abayMitigatingBiasFederated2020} propose two reweighing schemes.
In the first scheme, clients reweigh their local data independently,
while in the second scheme, the server computes the reweighing factors
based on statistics reported by the clients in a differentially private manner
(see \Cref{ssub:privacy:defenses:dp}).
Both schemes yield encouraging results on the Adult and COMPAS datasets.
\citet{duanAstraeaSelfBalancingFederated2019} propose another data preprocessing technique
for edge \gls{abb:fl} that aims to mitigate the impact of class imbalance.
The proposed method has two components: a global augmentation strategy,
and mediation-based rescheduling of the clients.
For data augmentation, the server queries the clients
for their local label distribution,
ordering them to augment classes with below-average frequency.
As for the second component, the server uses \emph{mediators}
which also serve as intermediate clients.
Each mediator runs asynchronous \gls{abb:fl} on the clients with the dual aim of
\begin{enumerate*}[label=(\roman*)]
  \item including all classes in the training set, and
  \item minimizing the entropy of the class distribution.
\end{enumerate*}
The server runs synchronous \gls{abb:fedavg} on the mediators.

\subsubsection{In-processing}\label{ssub:fairness:solutions:in}

In-processing techniques amend the learning algorithm itself.
As stated in~\Cref{sub:dq:solutions},
this family is significantly larger than the other two (at least in terms of literature).
In fact, all the techniques that deal with cooperative fairness are in this family,
along with many of the techniques that deal with social fairness.

\paragraph{Social fairness}\label{par:fairness:solutions:in:social}

Several works have proposed in-processing techniques
to ensure various notions of social fairness.
\citet{kamishimaFairnessAwareClassifierPrejudice2012}
introduce a regularization term that penalizes the \emph{``prejudice index''},
defined as the mutual information between
the classifier's prediction and the sensitive attribute.
In doing so, they aim to remove what they call \emph{``indirect prejudice''},
which corresponds to enforcing demographic parity in our terminology.
\citet{ezzeldinFairFedEnablingGroup2023} opt for a \gls{abb:gar} modification approach
to address the problem of group fairness in \gls{abb:fl}.
They propose updating client \(i\)'s coefficient \(\alpha_{i}\) based on
the difference between local fairness (as measured by a predetermined metric),
and the average fairness across all clients.
Testing against \gls{abb:fedavg} yielded better equal opportunity with modest accuracy loss.
A more detailed discussion of the literature on in-processing techniques for social fairness
can be found in~\cite{ferraguigSurveyBiasMitigation2021,mehrabiSurveyBiasFairness2022}.

\paragraph{Cooperative fairness}\label{par:fairness:solutions:in:coop}

Cooperative fairness strategies for \gls{abb:fl}
are as diverse as the definitions themselves.
To achieve good intent fairness, \citet{mohriAgnosticFederatedLearning2019}
devise \emph{agnostic} \gls{abb:fl}, an objective modification
which tries to solve a \(\min-\max\) problem
by running gradient descent-ascent on the parameters \(\theta\)
and the coefficients \(\alpha\).
\citet{raychaudhuryFairnessFederatedLearning2022} propose a \gls{abb:gar} modification
which converges provably to a model in the core.
They do so by assigning greater coefficients to clients
with lower \emph(relative) utility (normalized by the maximum utility).
Similarly, \citet{xuReputationMechanismAll2020} propose
a reputation-based \gls{abb:gar} modification wherein
clients with higher reputation get more weight.
On the theoretical side, \citet{donahueFairnessModelsharingGames2023}
establish bounds on both egalitarian and proportional fairness for certain games.
A thorough review of fair \gls{abb:fl} techniques
can be found in~\cite{%
  shiFairnessAwareFederatedLearning2023,%
  lyuCollaborativeFairnessFederated2020%
}.

\subsubsection{Post-processing}\label{ssub:fairness:solutions:post}

Examples of post-processing techniques for fair \gls{abb:ml} include
\citet{bolukbasiManComputerProgrammer2016}, which aims to produce fair word embeddings
by finding the dimensions that encode sensitive attributes and neutralizing them,
\citet{hardtEqualityOpportunitySupervised2016},
which seeks to enforce group fairness using the notion of a \emph{``derived predictor''},
and \citet{petersenPostprocessingIndividualFairness2021},
which targets individual fairness using graph Laplacian regularization.
None of these works are designed for the edge or \gls{abb:fl} settings.
In fact, to the best of our knowledge, no edge-specific
post-processing techniques have been proposed in the literature%
~\cite{ferraguigSurveyBiasMitigation2021}.

==> noise/solutions.tex <==
\subsection{Mitigating the effects of noise}\label{sub:noise:solutions}

Despite the few dissenting voices in the literature~\cite{%
  zengNoiseUsefulExploiting2021,%
  jafarigolParadoxNoiseEmpirical2023%
},
the prevailing consensus remains that label noise is a hindrance to the learning process~\cite{%
  alganImageClassificationDeep2021,%
  alganLabelNoiseTypes2020,%
  shanthiniTaxonomyImpactLabel2019,%
  barryImpactDataQuality2023%
}.
As such, many works have been dedicated to the remediation of its effects.
Multiple surveys have been conducted to review these works in the context of \gls{abb:ml}~\cite{%
  frenayClassificationPresenceLabel2014,%
  songLearningNoisyLabels2023,%
  hanSurveyLabelnoiseRepresentation2021,%
  yaoDeepLearningNoisy2019,%
  shanthiniTaxonomyImpactLabel2019%
},
but none have been conducted specifically for \gls{abb:fl} on the edge.
This is by no means the result of a lack of works in this area,
as the literature on the topic is vast and actively expanding~\cite{%
  tuorOvercomingNoisyIrrelevant2021,%
  yangClientSelectionFederated2022,%
  zhouFederatedLabelNoiseLearning2024,%
  jiFedFixerMitigatingHeterogeneous2024,%
  tamFederatedNoisyClient2023%
},
but rather the result of the novelty of the field.

In the remainder of this section,
we provide a brief overview of the state of the art
in the field of label noise mitigation,
focusing on the methods that are most relevant to the context of \gls{abb:fl} on the edge.
We adopt a taxonomy similar to the one we presented in Section~\ref{sub:dq:solutions},
except for the omission of the \emph{post-processing} category,
as we found no works that fall into it.

\subsubsection{Preprocessing}\label{ssub:noise:solutions:preprocessing}

The preprocessing of data for noise removal is known as \emph{data cleaning}.
\citet{yaoDeepLearningNoisy2019} divides data cleaning methods into two categories:
\begin{enumerate*}[label=(\roman*)]
  \item ad-hoc threshold measures, and
  \item prediction-based methods.
\end{enumerate*}
In the first  category, a heuristic metric is defined
and examples that exceed a certain cutoff value are considered noisy and removed.
\citet{gambergerNoiseEliminationInductive1996} introduced one such method
that uses \emph{model complexity} as the metric~\cite{yaoDeepLearningNoisy2019},
while \citet{pleissIdentifyingMislabeledData2020}
proposed another method that uses the \emph{area under the curve} instead.
The second category is more diverse and includes methods such as
classifiers~\cite{gambergerExperimentsNoiseLtering1999},
voting~\cite{brodleyIdentifyingMislabeledTraining1999},
and partitioning~\cite{zhuEliminatingClassNoise2003}.
While these methods are designed to work with traditional \gls{abb:ml} models,
\citet{maFederatedDataCleaning2021} proposed a \glsxtrfull{abb:smc}-based method
to privately and collaboratively clean the data in an \gls{abb:fl} system on the edge.

A common point of criticism for all these methods is that
they remove rather than correct the noisy labels.
In general, recovering the true labels is a very challenging (if not impossible) task.
This can be problematic if the data is scarce or if the noise is not uniformly distributed%
~\cite{yaoDeepLearningNoisy2019}.

\subsubsection{In-processing}\label{ssub:noise:solutions:inprocessing}

In-processing methods for removing label noise
are usually classified according to the element of the learning process they target.
In the context of general \gls{abb:ml},
This can be the loss function, the model architecture, or the optimizer%
~\cite{hanSurveyLabelnoiseRepresentation2021}.
\gls{abb:fl} on the edge adds two possible targets to this list,
namely the client selection protocol and the \gls{abb:gar}.
That being said, we could not find any works that target model architectures or optimizers
in the context of label noise-resilient edge \gls{abb:fl},
so we will focus on the other three elements,
directing the reader to referenced surveys
for information on their use in other contexts.

\paragraph{Loss function}\label{par:noise:solutions:inprocessing:loss}

Loss function modification strategies change the empirical risk function
by adding a regularization term that depends on the noise level
~\cite{%
  azadiAuxiliaryImageRegularization2016,%
  yuRegularizationPenaltyOptimization2022,%
  zhouFederatedLabelNoiseLearning2024%
},
modifying the loss function \(\ell\)~\cite{zhangGeneralizedCrossEntropy2018},
or by using a different distribution when taking the expectation
(also known as \emph{re-weighting})~\cite{liuClassificationNoisyLabels2016}.
A notable example of the latter is the work of \citet{chenRobustFederatedLearning2023},
which applies it to perform noise-robust \gls{abb:fl} on the edge.
A major strength of loss function modification strategies is
the existence of formal results establishing
their ability to produce near-optimal predictors under certain conditions,
as \citet{manwaniNoiseToleranceRisk2013} showed for \glspl{abb:dnn}%
~\cite{songLearningNoisyLabels2023}.

\paragraph{Client selection and aggregation}\label{par:noise:solutions:inprocessing:fl}

The methods discussed in this paragraph are specific to \gls{abb:fl},
%todo: consider moving this to the trust section
and have a meaningful amount of overlap with some defenses against
\emph{Byzantine attacks} (see \Cref{sub:trust:defenses}),
as those attacks can be seen as an intentional form of noise.
%todo: end
We discuss them jointly because they use the same strategies
to detect and evaluate noise.
They only differ in the way they handle the noisy clients (or data points):
either by reducing their weight in the aggregation process~\cite{xuReputationMechanismAll2020},
or by decreasing their probability of selection~\cite{yangClientSelectionFederated2022}.
% todo: these can mathematicall be seen as the same thing if modeled correctly
\citet{liSamplelevelDataSelection2021} took the latter approach,
using the magnitude of the gradient as a thresholding criterion.
In the same vein, \citet{tuorOvercomingNoisyIrrelevant2021} introduced
a selection mechanism that assesses the quality of a client's local dataset
by comparing its model to a benchmark model.
Almost identical to this is the work of \citet{taikDataQualityBasedScheduling2021},
which evaluates local models on a validation set instead.
\citet{chenDealingLabelQuality2020} on the other hand, took the former approach,
using a cross entropy-based metric to assign weights to the clients.


==> preamble/code.tex <==
\usepackage{minted}
% \usemintedstyle{native}
\setminted{%
  frame=lines,%
  framesep=2mm,%
  baselinestretch=1.2,%
  % bgcolor=DarkGray,%
  fontsize=\footnotesize,%
  linenos,%
  breaklines,%
}

\renewcommand{\listingscaption}{Code snippet}
\renewcommand{\listoflistingscaption}{List of code snippets}

==> preamble/hyperref.tex <==
\usepackage{hyperref}
\usepackage{cleveref}

\definecolor{CiteBlue}{HTML}{50A8C6}
\definecolor{Link}{named}{DarkBlue}

\makeatletter
\hypersetup{%
  colorlinks=true,
  linkcolor=Link,
  citecolor=CiteBlue,
  urlcolor=blue,
  pagecolor=red,
  pdfkeywords={Edge Computing, Machine Learning, Data Quality},
}

% Cleveref formats
\crefformat{principle}{principle.~#2#1#3}

==> trust/attacks.tex <==
\subsection{Byzantine attacks against federated learning}\label{sub:trust:attacks}

Being a distributed system, \gls{abb:fl} suffers from the Byzantine general problem.
This was first%
\footnote{%
  Previous works~\cite{suRobustMultiagentOptimization2016} highlight the problem
  in \gls{abb:ml}--adjacent contexts,
  but \citet{blanchardMachineLearningAdversaries2017} are credited
  for introducing it to \gls{abb:fl}.
}
pointed out by~\citet{blanchardMachineLearningAdversaries2017} in 2017,
who noted that the possibility of accidental or malicious misbehavior by clients
should be considered when designing \gls{abb:fl} systems.
Many subsequent works~\cite{%
  abyaneUnderstandingQualityChallenges2023,%
  yanDeFLDefendingModel2023,%
  el-mhamdiGenuinelyDistributedByzantine2020,%
  shejwalkarManipulatingByzantineOptimizing2021,%
  shiChallengesApproachesMitigating2022,%
  fangLocalModelPoisoning2020,%
  farhadkhaniEquivalenceDataPoisoning2022,%
  el-mhamdiCollaborativeLearningJungle2021,%
  el-mhamdiImpossibleSafetyLarge2023%
} have since explored the problem and potential solutions in depth,
resulting in a plethora of attacks and corresponding defenses.
This section provides an overview of Byzantine attacks,
while \Cref{sub:trust:defenses} discusses defense strategies.

Byzantine attacks can be classified according to various criteria~\cite{%
  jereTaxonomyAttacksFederated2021,%
  rodriguez-barrosoSurveyFederatedLearning2023,%
  xiaPoisoningAttacksFederated2023,%
  xiaSurveyFederatedLearning2021%
}, a common subset of which is
\begin{enumerate*}[label=(\roman*)]
  \item \emph{the attack level} (model or data),
  \item \emph{the goal} (degrading performance or inducing specific behavior), and
  \item \emph{the method} (the specific type of poison).
\end{enumerate*}
\Cref{fig:trust:taxonomies} illustrates two such taxonomies which include the three criteria
listed above, among others.
This section is structured according to the first criterion,
discussing model poisoning attacks in \Cref{ssub:trust:attacks:model},
and data poisoning attacks in \Cref{ssub:trust:attacks:data}.
\begin{figure}[hbt]
  \begin{center}
    \begin{subfigure}[b]{0.45\textwidth}
      \begin{center}
        \includegraphics[width=\textwidth]{assets/figures/images/lgft.jpg}
        \caption{According to level, goal, frequency, and time}%
        \label{fig:trust:lgft}
      \end{center}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.45\textwidth}
      \begin{center}
        \includegraphics[width=\textwidth]{assets/figures/images/lm.jpg}
        \caption{According to level and method}\label{fig:trust:lm}
      \end{center}
    \end{subfigure}
  \end{center}
  \caption{Taxonomy of Byzantine attacks~\cite{rodriguez-barrosoSurveyFederatedLearning2023}}%
  \label{fig:trust:taxonomies}
\end{figure}



\subsubsection{Model poisoning attacks}\label{ssub:trust:attacks:model}

In a model poisoning attack (or a gradient poisoning attack),
a Byzantine client generates its update by either modifying the honest update,
or crafting a malicious update from scratch.
In their seminal paper, \citet{blanchardMachineLearningAdversaries2017}
describe one such attack against \gls{abb:fedavg}.
Assuming the \gls{abb:gar} of \Cref{eq:fedavg} is used,
a Byzantine client \(j\) with a desired (arbitrary) model \(\tilde{\theta}\),
can send the update
\begin{equation}
  \theta_{j}^{(t)} = \frac{1}{\alpha_{j}} \tilde{\theta}
  - \sum_{i\neq j} \frac{\alpha_{i}}{\alpha_{j}} \theta_{i}^{(t)}
\end{equation}
to ensure that the global model \(\theta^{(t)}\) of the next round is \(\tilde{\theta}\).
A single attacker can thus hijack the global model under \gls{abb:fedavg}.
This can be used in a targeted manner (to induce a specific behavior),
or in an untargeted manner (to degrade the model's performance).

Subsequent works have explored other methods of implementing model poisoning attacks.
\citet{xieGeneralizedByzantinetolerantSGD2018} showcase a \emph{Gaussian attack},
where a Byzantine client samples its update from a normal distribution.
\citet{liRSAByzantineRobustStochastic2019} on the other hand, propose a
\emph{sign flipping attack}, where the attacker submits
a large negative multiple of the honest update.
Both of these attacks are untargeted.
Another untargeted attack introduced by~\citet{fangLocalModelPoisoning2020}
is more refined by virtue of its reliance on optimization techniques.
In this \emph{local model poisoning attack}, multiple Byzantine clients collude
to produce an update maximizing deviation from the honest gradient.

In contrast to these untargeted attacks, other authors have explored targeted ones
(also referred to as \emph{backdoor attacks}).
\citet{bagdasaryanHowBackdoorFederated2020} introduce a backdoor attack
where the attacker trains a local model on a mixture of correctly labeled and mislabeled data
to induce a backdoor, and then uses an attack similar to the one demonstrated by%
~\citet{blanchardMachineLearningAdversaries2017}
to replace the global model with its own.
Testing against \gls{abb:fedavg} was successful on
both image classification and language modeling tasks.

\subsubsection{Data poisoning attacks}\label{ssub:trust:attacks:data}

Data poisoning attacks are not specific to the edge.
\citet{chenTargetedBackdoorAttacks2017} proposed a targeted data poisoning attack against
\gls{abb:dl} in 2017.
Despite this lack of specificity,
data poisoning attacks are particularly relevant in the context of edge \gls{abb:fl},
due to the strong privacy requirements which usually prevent data inspection.
This family of attacks relies on the intuitive assumption
that compromising training data will compromise the model,
(inline with \Cref{princple:mq_is_dq}).
To mount a data poisoning attack,
a Byzantine client can either modify its features or its labels.
These two types of attacks are respectively known as
\emph{clean-label} and \emph{dirty-label} attacks~\cite{xiaPoisoningAttacksFederated2023}.

The most common form of dirty-label attack is the \emph{label-flipping attack}%
~\cite{xiaPoisoningAttacksFederated2023},
in which the attacker applies some permutation to the labels of its data%
~\cite{tolpeginDataPoisoningAttacks2020}.
This action is equivalent to applying a fixed, class-dependent label noise
(see \Cref{sub:noise:taxonomy}).
If this permutation is independent of the features
(or equivalently, if the noise is instance-independent),
the label-flipping is said to be \emph{static}, otherwise it is \emph{dynamic}%
~\cite{xiaPoisoningAttacksFederated2023}.
Attacks of this type can be targeted or untargeted,
depending on the structure of the permutation~\cite{xiaSurveyFederatedLearning2021}.

Clean-label attacks keep the labels intact,
opting instead to craft the features in a way that will mislead the model%
~\cite{xiaPoisoningAttacksFederated2023}.
This can be achieved in a multitude of ways.
An untargeted attacker may simply add random noise to the features%
~\cite{rodriguez-barrosoSurveyFederatedLearning2023},
while a targeted one may use a more sophisticated approach,
such as optimization techniques~\cite{shafahiPoisonFrogsTargeted2018}
or \glspl{abb:gan}~\cite{zhangPoisonGANGenerativePoisoning2021,zhangPoisoningAttackFederated2019}.

\subsubsection{Equivalence between data and model poisoning}\label{ssub:trust:attacks:equivalence}

A reasonably intuitive assumption on Byzantine attacks is that
model poisoning attacks are more effective than data poisoning attacks.
This can be rigorously justified by noting that data poisoning attacks
are trivially reducible to model poisoning attacks (by simply training on the poisoned data).
An equally valid observation is that data poisoning attacks are easier to mount,
and harder to detect (even in a centralized setting).
It is therefore reasonable to conclude that, by virtue of their respective limitations,
Byzantine attacks are not as dangerous as they may seem at first glance%
~\cite{shejwalkarBackDrawingBoard2022}.

\citet{farhadkhaniEquivalenceDataPoisoning2022} refute this claim by proving that
these two types of attacks are in fact equivalent.
Their proof is entirely constructive,
meaning that they provide an algorithm to construct an equivalent data poisoning attack
from any model poisoning attack.
This is done by essentially working backward,
generating a dataset by creating random instances
and labeling them according to the desired model.
Empirical evaluation yielded successful attacks against federated
linear regression and classification.

==> trust/defenses.tex <==
\subsection{Defense strategies}\label{sub:trust:defenses}

Given the potentially catastrophic impact of malicious clients,
defending against them is a critical concern in edge \gls{abb:fl}.
The literature on Byzantine-robust \gls{abb:fl} is vast and varied,
with a wide range of defense strategies.
In this section, we divide these strategies into two categories, namely,
\begin{enumerate*}[label=(\arabic*)]
  \item robust aggregation, which aims to \emph{mitigate} the impact of malicious clients
        by making the \gls{abb:gar} less sensitive to manipulation, and
  \item client selection, which focuses on \emph{detecting} malicious clients
        to either exclude them or reduce their selection probability.
\end{enumerate*}


\subsubsection{Robust aggregation}\label{ssub:trust:defenses:aggregation}


Robust aggregation functions are historically the first defense against Byzantine clients,
one having already been proposed in the seminal work%
~\cite{blanchardMachineLearningAdversaries2017}.
Since then, many other robust \glspl{abb:gar} have been proposed.
Many attacks specifically targeting them have also appeared in what has become an arms race.
In this section, we provide a brief overview of robust \glspl{abb:gar}.
Following~\cite{xiaSurveyFederatedLearning2021}, we divide them into three categories:
\begin{enumerate*}[label=(\arabic*)]
  \item score-based,
  \item median-based, and
  \item distance-based.
\end{enumerate*}
The reader can refer to~\cite{%
  fangLocalModelPoisoning2020,%
  wuToleratingAdversarialAttacks2021,%
  shiChallengesApproachesMitigating2022,%
  shejwalkarBackDrawingBoard2022%
}
for a more comprehensive overview of robust aggregation.

\paragraph{Score-based aggregation}\label{par:trust:defenses:aggregation:score}

This type of robust \gls{abb:gar} assigns a score to each update
and chooses the update with the highest (or lowest) score as the final aggregation.
Krum, the first robust \gls{abb:gar}~\cite{blanchardMachineLearningAdversaries2017},
is an example of a score-based aggregation function.
It scores each update vector based on the sum of squared distances
to a set of its closest neighbors
(the number of neighbors depends on the fraction of Byzantine clients)
and selects the vector with the lowest score.
In this way, Krum is able to tolerate \(\sim 1/2\) Byzantine clients.
However, Krum's inability to combine updates from different clients is a significant limitation.
To address it, multi-Krum~\cite{blanchardMachineLearningAdversaries2017}
interpolates between the Krum and \gls{abb:fedavg},
preserving robustness against \(\sim 1/2\) Byzantine clients.
Kardam~\cite{damaskinosAsynchronousByzantineMachine2018}
and Bulyan~\cite{mhamdiHiddenVulnerabilityDistributed2018}
are two other score-based \glspl{abb:gar}.
The former applies ``filters'' to either accept or reject updates in an asynchronous setting,
achieving robustness against \(\sim 1/3\) Byzantine clients.
The latter can be applied to any existing \gls{abb:gar} to increase its robustness.
It is able to tolerate \(\sim 1/4\) Byzantine clients.


\paragraph{Median-based aggregation}\label{par:trust:defenses:aggregation:median}

Median-based aggregation functions rely on the fact that the median is robust to outliers,
which makes it a better location indicator than the mean for extreme distributions%
~\cite{minskerGeometricMedianRobust2015}.
Computing the median of a set of vectors is not trivial,
as the univariate median can be extended to the multivariate case in many ways,
the most straightforward of which is coordinate-wise median
~\cite{yinByzantineRobustDistributedLearning2018}.
Other approaches include the geometric median~\cite{minskerGeometricMedianRobust2015},
which is provably (approximately) strategy-proof%
~\cite{el-mhamdiStrategyproofnessGeometricMedian2023},
the mean around median, and marginal median~\cite{xieGeneralizedByzantinetolerantSGD2018}.


\paragraph{Distance-based aggregation}\label{par:trust:defenses:aggregation:distance}

\glspl{abb:gar} in this category rely on the Euclidean \((\ell^{2})\) distance
to detect and exclude outliers.
Examples of such \glspl{abb:gar} include FABA~\cite{xiaFABAAlgorithmFast2019},
which iteratively removes the update with the largest distance to the mean,
\gls{abb:ios}~\cite{wuByzantineResilientDecentralizedStochastic2023},
an extension of FABA that works in a decentralized setting,
FoolsGold~\cite{fungMitigatingSybilsFederated2020},
which relies on cosine similarity to detect outliers in an asynchronous setting,
trimmed mean~\cite{yinByzantineRobustDistributedLearning2018},
which removes the tails of the distribution before computing the mean,
and Sniper~\cite{caoUnderstandingDistributedPoisoning2019},
which relies on the distance graph to detect outliers.

\subsubsection{Client selection}\label{ssub:trust:defenses:selection}

In contrast to robust aggregation, which aims to \emph{tolerate} Byzantine clients,
client selection strategies aim to \emph{detect} them (for total or partial exclusion).
This is implemented by allowing selection probabilities
to depend on the history of client behaviors,
assigning higher probabilities~\cite{raiClientSelectionFederated2022}
or weights~\cite{chenDealingLabelQuality2020}
to clients with a better track record.
The most common approach is to use a \emph{trust} score or \emph{reputation} value
to quantify the reliability of each client~\cite{%
  byabazaireUsingTrustMeasure2020,%
  chuprovReputationTrustModels2020%
}.
% (accounting for both the quality of the data and the behavior of the client).
Computing this score requires the ability to detect malicious behavior,
which is a challenging problem in and of itself.
The remainder of this section is dedicated to the discussion of
Byzantine behavior detection strategies.

\paragraph{Centralized testing}\label{par:trust:defenses:selection:centralized}

These strategies compare each client against the behavior of the rest,
giving lower scores to clients with significantly detrimental behavior.
In this vein, \citet{taikDataQualityBasedScheduling2021} propose a reputation-based
client selection scheme where reputation scores are computed by comparing self-reported
local accuracies with the average accuracy on one hand (to detect data quality issues),
and the accuracy of the proposed model on a common validation set on the other hand
(to detect dishonest clients).
The server then selects clients by solving an instance of the \knapsack{} problem
to maximize the total reputation score within a communication budget.

Similarly, \citet{xuReputationMechanismAll2020} propose to assign reputation scores
to clients based on comparison with the global model.
More precisely, the reputation of a client at round \(t\)
is computed as an exponential moving average of the cosine similarity between
its update and the aggregated update at round \(t\).
Instead of being used for client selection, reputation scores are used as
aggregation coefficients in the next round.

Alternatively, \citet{liSamplelevelDataSelection2021} present a client selection strategy
based on \gls{abb:dq} (assuming honest-but-curious clients).
Clients are assigned an ``importance'' score based on the \(\ell^{2}-\)norm of their update
(or the magnitude of their local loss).
A client is then selected with a probability proportional to its importance score.
This is almost diametrically opposed to previously discussed strategies%
~\cite{taikDataQualityBasedScheduling2021,xuReputationMechanismAll2020},
in that it favors rather than penalizes outliers.
The rationale is that local datasets on which the global model performs poorly,
are precisely the ones it needs to be trained on to improve its \emph{true risk}.
That being said, the authors do acknowledge that abnormally large updates
are likely to be the result of low data quality,
which we note can be intentional (Byzantine) as well as unintentional (noise).
To address this, they propose a threshold on the importance score,
beyond which a data point is discarded as noise.

\paragraph{Proof of learning}\label{par:trust:defenses:selection:PoL}

In 2021, \citet{jiaProofofLearningDefinitionsPractice2021}
introduced the concept of a \gls{abb:PoL},
a mechanism for a party to prove that it has trained a model.
This can be used to claim ownership of said model,
or, crucially for edge \gls{abb:fl}, to allow the server to verify an update
is the result of a legitimate training process.
This is done by periodically providing the server with a \gls{abb:PoL},
consisting of a model update and the data point used to produce it,
signed, timestamped, and encrypted to prevent spoofing and replay attacks.
Recent work has extended this concept using zero-knowledge proofs
to allow for the verification of the update
without revealing any information about the data%
~\cite{gargExperimentingZeroKnowledgeProofs2023}.
